PrivacyGuard: Enforcing Private Data Usage Control with Blockchain and Attested Off-chain Contract Execution

The abundance and rich varieties of data are enabling many transformative applications of big data analytics that have profound societal impacts. However, there are also increasing concerns regarding the improper use of individual data owner's private data. In this paper, we propose PrivacyGuard, a system that leverages blockchain smart contract and trusted execution environment (TEE) to enable individual's control over the access and usage of their private data. Smart contracts are used to specify data usage policy, i.e., who can use what data under which conditions and what analytics to perform, while the distributed blockchain ledger is used to keep an irreversible and non-repudiable data usage record. To address the efficiency problem of on-chain contract execution and to prevent exposing private data on the publicly viewable blockchain, PrivacyGuard incorporates a novel TEE-based off-chain contract execution engine along with a protocol to securely commit the execution result onto blockchain. We have built and deployed a prototype of PrivacyGuard with Ethereum and Intel SGX. Our experiment result demonstrates that PrivacyGuard fulfills the promised privacy goal and supports analytics on data from a considerable number of data owners.

==> figures/Algorithm_contractExecutionEnclave.tex <==



% 
%  Contract Execution Enclave
% 
\begin{algorithm}
\algfootnote
\begin{centering}
\caption{Program for Off-chain Contract Execution ($OCEP_{enclave}$)}
\label{alg.cee}
\end{centering}

% when data is received, it is encrypted by privacy guard with appropriate data encryption key and placed in the Cloud
\BlankLine
\Fn{Initialize ($Req_{DataOp}$)}{
	parse request as ($DC$,$DO$,$Op$,data,sig)				\;
	send $Req_{DataOp}$ and $\sigma_{att}$ to $DO$ 			\;
	send $Req_{DataOp}$ and $\sigma_{att}$ to $DC$ 			\;
}

% when privacy guard receives the request to use data
\BlankLine
\Fn{OnDataOpeationApproval (approval)}{
	Parse approval as (pk$_{approver}$, OpUid, sk$_{op}$, sig$_{approver}$)		\;
	\If{$\neg$SigVerify(sig$_{approver}$)}
	{terminate \;}
	\If{approver$_{DC}$}
	{sk$_rec \leftarrow$ sk$_{op}$}
	\If{approver$_{DO}$}
	{sk$_dec \leftarrow$ sk$_{op}$}
% Until we figure out what T is used for, let's keep that comment out
	% Assert clock() $ \geq T.min $;			\;
	% Assert clock() $ \leq T.max $;			\;	
	\If{$\neg$ approval$_{DO}$ $\lor$ $\neg$ approval$_{DC}$}
	{terminate \;}
	C$_{Data} \leftarrow $ loadFromStorage  				\;
	Data $\leftarrow \Sigma$.Decrypt(C$_{Data}$,sk$_dec$) 	\;
	result := Op(Data)										\;
	$g_{rec}$ := $G_{max}$									\;
	$\sigma$ := $\Sigma$.Sign(sk$_{dc}$)					\;
}


% \caption{The Contract Execution Enclave Program}
\end{algorithm}



==> figures/Algorithm_dataBroker.tex <==
\begin{algorithm}[h]
\algfootnote
\begin{centering}
\caption{Program for \db TEE}
\label{alg.db.tee}
\end{centering}

% when privacy guard receives the request to use data, it needs to 
% 1. make sure that the request is legit by checking the access control mechanism, it could be the block chain or a simple table in the enclave
% 2. if the access request is legit, it should check to make sure that there enough deposit made by the data consumer, but how do we do that in the block chain ?
% 3. it should verify the remote attestation result of the execution enclave
% 4. 
\BlankLine
\Fn{OnRecvDataUseRequest (request)}{
	% Parse request as (pk$_{DC}$, data, op, $\sigma_{att}[CExeProg_{enclave}]$, pk$_{ce}$, $T$);		\;
	Parse request as (pk$_{DC}$,data, op, $\sigma_{att}$, pk$_{ce}$, $T$)		\;
	% checkAccessRight(pk$_{DC}$,data)$\neq$true
	\tcc{verify the access right on the contract}
	\If{$\neg$CheckAccessRight(pk$_{DC}$,data)}
	{terminate \;}
	% \tcc{verify the attestation on contract execution enclave}
	\If{$\neg$VerifyAttestation(pk$_{DC}$,$\sigma_{att}[CExeProg_{enclave}]$)}
	{terminate \;}
	transmit(list($k_{data}$),Addr$_{CEE}$) \;
	storeDataAccessOffChainForAllUsers() \;
	storeDataAccessOnChainForTheContractedUsage() \;
	% Assert clock() $ \geq T.min $			\;
	% Assert clock() $ \leq T.max $			\;	
	% FIXME: Look into the details of the gas manipulation 
}

\BlankLine
\Fn{OnRegisteringForData (request)}{
	% Parse request as (pk$_{DC}$, data, op, $\sigma_{att}[CExeProg_{enclave}]$, pk$_{ce}$, $T$);		\;
	Parse request as (pk$_{DC}$, link$_{data}$, op list, sk$_{data}$,$\sigma_{att}$, $T$)		\;
	\If{$\neg$CheckDataRegisterOnChain(pk$_{DC}$,link$_{data}$)}
	{terminate \;}
	% \tcc{verify the attestation on contract execution enclave}
	\If{$\neg$VerifyData(link$_{data}$,sk$_{data}$)}
	{terminate \;}
	completeOnChainDataRegister()   \;
	% Assert clock() $ \geq T.min $			\;
	% Assert clock() $ \leq T.max $			\;	
	% FIXME: Look into the details of the gas manipulation 
}


\BlankLine
\Fn{OnCompletionOfDataTransaction (request)}{
	parse request as ($k_{result}$)

}


\end{algorithm}

==> sec-securityanalysis.tex <==
\section{Security Analysis}
\label{sec:secAnalysis}

% TODO: There might be more attacks than what we currently have here, do some more thinking
%  Also what is the best logical way to present this ?

% \sysname has two key components, blockchain in the control plane and TEE in the data plane. 
% The security properties of these two primitives have received significant amount of attentions recently~\cite{van18foreshadow,xu2015controlled,zhang2016case,luu2016making,kogias2016enhancing,zhang2016town,hawk,ekiden}. 
% In the discussion below, the focus will be on issues in harmonizing TEE and blockchain. For 
In \sysname, a single on-chain contract function is partitioned into multiple functions both on and off chain using the proposed off-chain execution technique. This technique has opened new avenues for adversaries that are not previously available on conventional blockchain platform.
% Furthermore, with the assumption that attacker will not be able to compromise enough nodes in the blockchain network to affect consensus, our analysis will examine the implication of adversarial control of off-chain computing platform, which is centralized according to our design of `local consensus'. 

\subsection{Exploiting Control of Cloud Platform}

Off-chain contract execution significantly reduces the computation load on the blockchain network, but at the same time provides a single point of failure if the adversary is able to compromise the cloud platform.
% \subsubsection{Denial of Service}
During the execution of the off-chain contract stage, the adversary can stop the program at any time, and drop or reorder any message. However, he cannot tamper with the content of the network message as long as the connection is secured. Anticipating the execution of the data contract can be halted by the adversary at any stage, our design on the data contracts allows any party to abort the data transaction without incurring financial loss. 
%
It should however be noted that, although we expect a trusted source to examine the data analytic program, the adversary may still attempt to launch side channel attack or directly exploit a software vulnerability in program within the SGX enclave, which is out of the scope of this paper. 
% It should however be noted that, although we expect a third party to examine the program, implementations are often imperfect. 
Therefore due to the use of TEE 
% to provide secure execution environment for 
for hosting the data analytic program, our system inherits vulnerabilities of implementation of both the TEE and the data analytic program. 

% \subsubsection{Manipulating Data Broker Network}


% \subsection{Exploiting the Incoherence Between Data Plane and Control Plane in Result Commitment}
\subsection{Exploiting the Incoherence Between Data and Control}

% There are three main players in the last stage (result commitment and release) of the data operation contract: \mdo, \mdb and the Cloud. 
Ideally, the release of the data and the deposit should be an atomic decision. 
However, with the separation of control plane and the data plane, these operations may become inherently non-atomic. 
% This is further complicated by the fact that there is lack of availability guarantee for the TEE technology we choose to implement \sysname, Intel SGX. Transactions on blockchain is used to signal the completion of the data operations and enable the completion of the financial transaction for the data use. On the other hand, this does not necessarily guarantee the delivery of result to the data consumer who has already paid for the service using the control plane operation on the blockchain. 
There are several ways an adversary can attack our result commitment and release protocol shown in Fig. \ref{fig.offchainexe}. We assume the \mdb is used.

% \textbf{\emph{DO} controls the cloud:}
\textbf{\emph{DB} controls the cloud:}
The \mdb, assuming compromised by a malicious \mdo, may attempt to complete the data transaction without having \tcee upload the result even \mdc has paid the deposit. Using the control of the Cloud platform, the \mdb can either maliciously modify the data operation result or he can simply deny the output of results. In \sysname, this attack is thwarted by having the \textit{ComputationComplete} contract function to enforce the result commitment before completing the data transaction. 

% The TEE receiving the success return from the malicious operating system will happily close without the ability to detect the result has been altered or deny. 

% \subsubsection{\mdc controls the Cloud}
% In this case, the \mdc may attempt to get the result without completing the transaction (i.e the payment). Assuming control of the Cloud infrastructure, an adversary can simply intercept the commitment message from the TEE to the contract on blockchain. Using the malicious OS, the adversary can forge a success publication response from the blockchain. However, without the observing the commitment message from blockchain, the \mdo or \mdb will never follow on the state machine to release the result via \textit{CompleteDataTransaction()} contract call. Therefore, the adversary, \mdc in this case, will not be able to gain any unfair advantage.
% If the data consumer is malicious and data broker is hosted in a trusted container in the Cloud, and the data consumer is able to compromise the Cloud platform where data broker is hosted. The data consumer might be able to manipulate blockchain network traffic in attempt to mislead the \mdb to believe that \textit{ComputationComplete()} has been invoked in the blockchain. When the data broker invokes \textit{CompleteTransaction()}, the function would fail in that data broker contract, he would not get the payment because the contract never receive the \textit{ComputationComplete()} message. However, the adversary, the data consumer would still be able to obtain the result disclosure key $K_{result}$ from the transaction itself, despite the failure in completing the transaction. Based on the deployment strategy of data broker, it is often not possible for data consumer to completely influence data broker's view on the blockchain state. Notably, our implementation makes the assumption that complete adversarial manipulation of data broker's blockchain state is impossible, because we assume data broker is able to establish secure connection with at least one honest node in the network. Furthermore, we can also reasonably remove this assumption by adding functionality to verify the proof of publication in data broker.

\textbf{\emph{DC} controls the cloud:}
% Under unlikely circumstances, 
If a malicious \mdc is powerful enough to compromise the platform which \mdb and \mdo are running on, he might be able to capture the last commitment message to get the result release key, but never forward the blockchain invocation message to the network. This way, the \mdc can obtain the result without completing the payment. However, with an increasing number of nodes accepting transaction broadcasts in secure manner, even though the adversary might be able to block all the connection, he cannot break the secure connection by launching man-in-the-middle attack. This attack is thwarted by our system sending the \textit{CompleteTransaction} message to a collection of transaction recipients in secure channels. The \textit{CompleteTransaction} message, which contains the result release key, will only be transmitted if the secure channel can be established. Therefore the adversary would have to block all of the traffic, otherwise he cannot block the transaction broadcasts. When all the network connections are blocked, the result will never be released, which is not a problem for \mdb and \mdo. When the adversary can only block a subset of the result broadcast messages, the data transaction will continue to complete.
% and thus is not an issue either. 
% Furthermore, it is also possible to add functionality to verify the proof of publication in data broker instead of relying on broadingcast via secure channel. 

